Exploring How Generative Adversarial Networks Learn Phonological Representations

This paper explores how Generative Adversarial Networks (GANs) learn representations of phonological phenomena. We analyze how GANs encode contrastive and non-contrastive nasality in French and English vowels by applying the ciwGAN architecture (Begus 2021a). Begus claims that ciwGAN encodes linguistically meaningful representations with categorical variables in its latent space and manipulating the latent variables shows an almost one to one corresponding control of the phonological features in ciwGAN's generated outputs. However, our results show an interactive effect of latent variables on the features in the generated outputs, which suggests the learned representations in neural networks are different from the phonological representations proposed by linguists. On the other hand, ciwGAN is able to distinguish contrastive and noncontrastive features in English and French by encoding them differently. Comparing the performance of GANs learning from different languages results in a better understanding of what language specific features contribute to developing language specific phonological representations. We also discuss the role of training data frequencies in phonological feature learning.

==> section/_09_review.tex <==
\clearpage
\section{Review}
\subsection{Reviewer \#1}


\paragraph{1}Presentation of the dataset creation, the methodology and the results are often obscure and require several readings.

\paragraph{2}The discussion is short and does not address an in-depth analysis of the observed correlation: what do we learn from it in a linguistic perspective, to what extent the approach is generalizable to other linguistic features?

\paragraph{3}At a more detailed level, a more precise analysis of the latent space is necessary, and figures (especially figures 2, 4, 5) should be more precisely commented.

\begin{table}[htbp]
\centering
\begin{tabular}{|*{2}{c|}} 
 \hline
Soundness & 4 \\ \hline
Excitement & 3.5\\\hline
Confidence & 3\\\hline
Reproducibility&3\\\hline
\end{tabular}
\end{table}


\subsection{Reviewer \#2}
\paragraph{1}The experiment is limited to a single phenomenon, and only take in consideration data from 2 distinct datasets. Some details of the experiments could be better described.

\begin{table}[htbp]
\centering
\begin{tabular}{|*{2}{c|}} 
 \hline
Soundness & 4 \\ \hline
Excitement & 3.5\\\hline
Confidence & 3\\\hline
Reproducibility&4\\\hline
\end{tabular}
\end{table}

\subsection{Reviewer \#3}

\paragraph{1}I believe the authors are implying (around line 117) that their results apply to (Ciw)GANs in general, i.e. for some encoder to a downstream task. However, their experimental design is very narrow, focusing only on the case where stimuli curated to contrast the phonological feature in question (e.g. segments of vowel-consonant pairs) are used to train the model. It is not obvious to me that these results will generalize beyond this very constrained task.


\paragraph{2}Question A: In response to my concerns about generalizability above, I would like to hear a more detailed account of the "big picture" of this paper from the authors. How are the results expected to generalize? Maybe, instead, that the model can perform phonological feature learning (or cannot, as the case may be) will lead to a certain form of research?
\paragraph{3}Question B: The paper details where the regression's dependent variable came from in the case of English: an auxiliary CNN trained on TIMIT. Where did it come from in the case of French? If the same CNN was used for French, how were nasal consonants separated from nasal vowels?



\paragraph{5}Question C: I am unclear on why it's so important that one or more of these variables independently control for nasality. Aren't we only interested in if it is separable in the latent space? Perhaps some eigendecomposition would be more fruitful, or an explanation provided why it wouldn't be.



\paragraph{6}Missing References: van der Oord's CPC paper might be relevant for its similar categorical prediction task: "Representation Learning with Contrastive Predictive Coding"
\paragraph{7}Typos, Grammar, Style, and Presentation Improvements
\begin{enumerate}
    \item Some additional, high-level signposting about the experiments to be perfomed might help to keep things straight.
    \item A more careful description of the categorical variables in section 3 would have helped as well. 
    \item A line summarizing the mechanism for choosing the latent variables to examine would also be helpful. 
    \item Removing the raw signal portion of figure 3 would grant some space.
\end{enumerate}

\begin{table}[htbp]
\centering
\begin{tabular}{|*{2}{c|}} 
 \hline
Soundness & 3 \\ \hline
Excitement & 2.5\\\hline
Confidence & 3\\\hline
Reproducibility&3\\\hline
\end{tabular}
\end{table}
\subsection{Reviewer \#4}


\paragraph{1}	it does focus on a single allophone across two languages. It is unsure to what extent the conclusions could be generalised to other phonemes or languages. In order to be certain that GANs reliably encode contrastiveness versus allophonic phenomena, more allophones and languages would have to be tested. 
\paragraph{2}	There are also many points in the manuscript where the phrasing is unclear and makes it difficult to follow the argument.
\paragraph{3}	Question A.    Could the authors expand on why autoencoders are not able to learn one-to-one mappings as opposed to GANs? This wasn't clear to me. In general, while the authors make claims about the shortcomings of current models they do not clarify precisely what they are.

\paragraph{4}	Question B.    What do the authors mean by ‘generate audio that carries specific lexicon features'? Also, is lexical knowledge necessary for building phonological representations? (I believe this is linked to the model's ‘Q network' but it should be made clearer what the components are and what they do). 


\paragraph{5}	Question C.    The paper would greatly benefit from giving some example lexical items from the dataset in both languages 
\paragraph{6}	Question D. Could the authors provide the GAN parameters and explain the model architecture further 


\paragraph{7}Typos, Grammar, Style, and Presentation Improvements

l199: ‘an autoencoder'

l201: ‘output values'

l270: ‘They manually label'

l308: ‘for the English experiment'

l389: ‘a lower amplitude'

l399: ‘do not have'

l418: ‘they also'

\begin{table}[htbp]
\centering
\begin{tabular}{|*{2}{c|}} 
 \hline
Soundness & 4 \\ \hline
Excitement & 4\\\hline
Confidence & 3\\\hline
Reproducibility&3\\\hline
\end{tabular}
\end{table}
